Accounting for Climate Change in Extreme Sea Level Estimation

Extreme sea level estimates are fundamental for mitigating against coastal flooding as they provide insight for defence engineering. As the global climate changes, rising sea levels combined with increases in storm intensity and frequency pose an increasing risk to coastline communities. We present a new method for estimating extreme sea levels that accounts for the effects of climate change on extreme events that are not accounted for by mean sea level trends. We follow a joint probabilities methodology, considering skew surge and peak tides as the only components of sea levels. We model extreme skew surges using a non-stationary generalised Pareto distribution (GPD) with covariates accounting for climate change, seasonality and skew surge-peak tide interaction. We develop methods to efficiently test for extreme skew surge trends across different coastlines and seasons. We illustrate our methods using data from four UK tide gauges.

==> Sections/RL_est.tex <==
To understand how these trends in extreme skew surges would influence sea level return levels, we estimate high quantiles of the skew surge distribution function given in expression~\eqref{eqn::ss_model} but with our added trend parameters. For the rate parameter, we use Model~$R4$ (expression~\eqref{eqn::mod_lambda_ssnl_gmt}) with a separate GMT trend for each season, and for the scale we use Model~$S0$ of~\cite{DArcy22}, without a longer-term trend parameter. Then we find the difference between the 0.99, 0.999 and 0.999 quantiles of the skew surge distribution $F^{d,j,x,m}$ at $m=0$ and $m=1$, corresponding to a $1^\circ$C increase in GMT; we average the distribution function over all $d,j$ and $x$.

==> Sections/pooling.tex <==
Since there is overlap in the parameter estimates for $\hat\xi$ in the skew surge model of \cite{DArcy22}, we now suggest sharing information about this parameter across the study sites, assuming they are independent. In this section, we add a prior distribution to the shape parameter and investigate if this improves model fit. Then we present a framework to check if the longer-term trends discussed in Section~\ref{sec::trends} for the scale and rate parameter could also be pooled across sites. We discuss the results in Section~\ref{sec::pooling_results}.

In~\cite{Darcy22} they add a prior distribution to the shape parameter; this is a Normal$(0.0199, 0.0343^2)$ based on site-specific shape parameters for the entire UK National Tide Gauge Network used in \cite{CFB2018}. We fit this model using a penalised-likelihood framework and investigate if this improves model fit. Parameter estimates are given in Table~\ref{tbl:shape_param_ests} with 95\% confidence intervals. We find that incorporating this prior information reduces both AIC and BIC by 15.~\cite{Darcy22} demonstrate a significant a reduction in sea level return level estimation at the highest return periods when this prior penalty is added to the skew surge model. In Section~\ref{sec::pooling_results}, we refit all of the models in Section~\ref{sec::trends} to check if our results change.

\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccc}
        \hline
         & Heysham & Lowestoft & Newlyn & Sheerness\\ \hline
         No pooling & 0.0049 (-0.044, 0.054) & 0.024 (-0.023, 0.071) & -0.037 (-0.071, -0.003) & 0.033 (-0.033, 0.099)\\
         Prior on shape & 0.019 (-0.021, 0.059) & 0.014 (-0.024, 0.052) & -0.027 (-0.058, 0.004) & 0.008 (-0.039, 0.054) \\
         Common shape & \multicolumn{4}{c}{-0.005 (-0.028, 0.018)} \\
    \end{tabular}
    }
    \caption{Shape parameter estimates for the extreme skew surge model of~\cite{DArcy22}.}
    \label{tbl:shape_param_ests}
\end{table}

==> Sections/threshold.tex <==
%%%%%%%%%%%%%%% EDIT FROM JON %%%%%%%%%%%%%%
Threshold choice for the GPD and other tail models for identically distributed univariate extremes has been a major area of publications for much of the last 40 years. It is not surprising that there are a number of different perspectives for picking a systematic threshold selection criteria in our temporally non-stationary spatial context. 


One option is to have a threshold $u(t,\boldsymbol{\site})$ that varies over time and site computed from a given quantile, e.g., $u(t,\boldsymbol{\site})=\hat{q}_o^{(\tau)}(t,\boldsymbol{\site})$, for some choice of $\tau$. However, it is well known that it is difficult to account for the uncertainty in the threshold selection in extreme value inference (\citealp{Wadsworth2012a}, \citealp{Scarrott2012}, \citealp{Northrop2017a}). 

Since here it is the temporal change in extreme events which is of most interest, it seems problematic to allow the threshold to vary over time. Instead we choose the threshold to be constant over time   $u(\boldsymbol{\site})$; a choice discussed further in Section~\ref{SEC7}.

For univariate temporally non-stationary problems \cite{Eastoe2009} propose pre-processing the data using models fitted to the body of the distribution before modelling the extremes of the residuals with a constant threshold. Another approach is to use a conditional quantile \citep{Northrop2011}. As noted in Section~\ref{sec:above}
it is difficult to account for the uncertainty in the threshold selection yet estimating this temporal change is our focus. We are pleased to see that even with our temporally homogeneous threshold at each station we found very simple models for the GPD scale parameter and that the non-stationarity primarily affected just the threshold exceedance probability - with the uncertainty of this easily captured through our bootstrapping procedure. More generally, the signal to noise ratio is critical in determining whether non-stationarity is accounted for in selecting the set of ``extreme data" to analyse.


==> header.tex <==
% HEADER

% a % sign means the rest of the line is ignored
% modify page size and spacing at end

% PREAMBLE
\usepackage{graphicx}
\usepackage{natbib}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{url}

% format for environments follows
% \newenvironment{name}{starting text}{finishing text}

\newenvironment{proof}{\begin{trivlist} \item[]
{\bf Proof.}}{\nolinebreak
\hfill \rule{2mm}{2mm} \end{trivlist}}

% matrix and determinant environments follow
\newenvironment{mat}{\left[ \begin{array}}{\end{array} \right]}
\newenvironment{deter}{\left| \begin{array}}{\end{array} \right|}

% controls the way equations are numbered
%\numberwithin{equation}{section}
% format for lists follows
% \begin{list}{label for items}{declarations} items in list \end{list}

% lista, listr, listar, listq are list environments with
% small letters, small roman numerals, arabic numerals and no item labels
\newcounter{ctr}
\newenvironment{lista}{\begin{list}{(\alph{ctr})}%
{\usecounter{ctr}
\setlength{\itemsep}{0mm} \setlength{\topsep}{-2mm}
\setlength{\leftmargin}{3em}}}{\end{list}}

\newcounter{ctr1}
\newenvironment{listr}{\begin{list}{(\roman{ctr1})}%
{\usecounter{ctr1}
\setlength{\itemsep}{0mm} \setlength{\topsep}{-2mm}
\setlength{\leftmargin}{3em}}}{\end{list}}

\newcounter{ctr2}
\newenvironment{listar}{\begin{list}{\arabic{ctr2}.}%
{\usecounter{ctr2}
\setlength{\itemsep}{0mm} \setlength{\topsep}{-2mm}
\setlength{\leftmargin}{3em}}}{\end{list}}

\newenvironment{listq}{\begin{list}{}%
{
\setlength{\itemsep}{0mm} \setlength{\topsep}{-2mm}
\setlength{\leftmargin}{3em}}}{\end{list}}

% environments for an example, examples or exercises follow

\newenvironment{example}{\begin{list}{}%
%{\addtocounter{subsection}{1} \item[] {\bf Example \thesubsection}%book
%{\addtocounter{subsubsection}{1} \item[] {\bf Example \thesubsubsection}%art
{\addtocounter{definition}{1} \item[] {\bf Example \thedefinition}
\setlength{\itemsep}{0ex} \setlength{\topsep}{0ex}
\setlength{\leftmargin}{3em}} \item }{\end{list}}

\newcounter{ctr3}
\newenvironment{examples}{\begin{list}{\arabic{ctr3}.}%
{\usecounter{ctr3} \addtocounter{definition}{1} \item[]
{\bf Examples \thedefinition }
%{\usecounter{ctr3} \addtocounter{subsection}{1} \item[] %book style
%{\bf Examples \thesubsection }                          %book style            %{\usecounter{ctr3} \addtocounter{subsubsection}{1} \item[] %article style
%{\bf Examples \thesubsubsection }                          %article style
\setlength{\itemsep}{0ex} \setlength{\topsep}{0ex}
\setlength{\leftmargin}{3em}}}{\end{list}}

\newenvironment{exercises}{\begin{trivlist} \item[]
{\bf Exercises} \begin{enumerate}}{\end{enumerate} \end{trivlist}}

% format of new theorem-like environments follows
% \newtheorem{name}{printed caption}[name of environment in which numbered]
% or
% \newtheorem{name}[numbered as another theorem type]{printed caption}

%\newtheorem{definition}{Definition}[section]    %for book style
\newtheorem{definition}{Definition}[subsection] %for article style
\newtheorem{theorem}[definition]{Theorem}
\newenvironment{theorem*}[1]{{\bf Theorem #1} \begin{itshape}}{\end{itshape}}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{corollary}[definition]{Corollary}
\newenvironment{corollary*}[1]{{\bf Corollary #1} \begin{itshape}}{\end{itshape}}
\newtheorem{proposition}[definition]{Proposition}
\newenvironment{proposition*}[1]{{\bf Proposition #1} \begin{itshape}}{\end{itshape}}
\newtheorem{remark}[definition]{Remark}

% commands for number sets follow
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\LL}{\mathbb{L}}

% commands for extra mathematical symbols follow
\newcommand{\half}{\frac{1}{2}}
\newcommand{\third}{\frac{1}{3}}
\newcommand{\quarter}{\frac{1}{4}}
\newcommand{\isimp}{\Leftarrow}
\newcommand{\lsim}{\stackrel{<}{_\sim}}
\newcommand{\gsim}{\stackrel{>}{_\sim}}
\newcommand{\image}{\, {\rm im}\, }
\newcommand{\rank}{\, {\rm r}\, }
\newcommand{\domain}{\, {\rm dom}\, }
\newcommand{\adjoint}{\, {\rm adj}\, }
\newcommand{\signum}{\, {\rm sgn}\, }
\newcommand{\cosec}{\, {\rm cosec}\, }
\newcommand{\cis}{\, {\rm cis}\, }
\newcommand{\sech}{\, {\rm sech}\, }
\newcommand{\cosech}{\, {\rm cosech}\, }
\newcommand{\trace}{\, {\rm trace}\, }
\newcommand{\diag}{\, {\rm diag}\, }
\newcommand{\tri}{\, {\rm tri}\, }
\newcommand{\ud}{\, {\rm d} \kern-.015em }
\newcommand{\const}{\! {\rm const.}\; }


% the following commands need 1 or 2 arguments in { }
\newcommand{\real}[1]{{\rm Re}\left( #1 \right)}
\newcommand{\modulus}[1]{\left| \kern.05em #1 \kern.05em \right|}
\newcommand{\norm}[1]{\left\| \kern.05em #1 \kern.05em \right\|}
\newcommand{\inner}[1]{\left\langle \kern.05em #1 \kern.05em \right\rangle }
\newcommand{\recip}[1]{\frac{1}{#1}}
\newcommand{\seq}[1]{\left( #1 \right)}
\newcommand{\set}[1]{\left\{ #1 \right\} }
\newcommand{\spanof}[1]{\, {\rm span} \left\{ #1 \right\} }
\newcommand{\limit}[2]{\stackrel{\lim }{_{ #1 \to #2 }}}
\newcommand{\maxover}[1]{\stackrel{\max }{_{ #1 }}}
\newcommand{\minover}[1]{\stackrel{\min }{_{ #1 }}}
\newcommand{\dislim}[2]{\renewcommand{\arraystretch}{0.8}
\begin{array}{c}\lim \\ #1 \to #2 \end{array}}
\newcommand{\pdif}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pddif}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\dif}[2]{\frac{\ud #1}{\ud #2}}
\newcommand{\ildif}[2]{{\rm d} #1/{{\rm d} #2 }}
\newcommand{\ilpdif}[2]{\partial #1/{\partial #2 }}
\newcommand{\ilpddif}[3]{\partial^2 #1/{\partial #2 \partial #3}}
\newcommand{\seconddif}[2]{\frac{\ud^2 #1}{\ud #2^2}}
\newcommand{\bm}[1]{\mbox{\protect\boldmath $ #1 $}}
\newcommand{\bmzero}{\mbox{\bf 0}}
\newcommand{\pick}[2]{\renewcommand{\arraystretch}{0.6}
\left( \kern-.4em \begin{array}{c} #1 \\ #2 \end{array} \kern-.4em \right) }
\newcommand{\e}[1]{{\textrm{e}}^{#1}}
\newcommand{\cov}[1]{\, {\rm cov}\left( #1 \right) }
\newcommand{\var}[1]{\, {\rm var}\left( #1 \right) }
\newcommand{\PP}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\EE}[1]{\mathbb{E} \left( #1 \right)}

% SET PAGE SIZES IN FOLLOWING

\pagestyle{plain}
%\pagestyle{empty}
%\pagestyle{headings}

%\setlength{\textwidth}{6.5in}
\setlength{\textwidth}{7.0in}
%\setlength{\textwidth}{10.5in} 

%\setlength{\textheight}{9.0in}
%\setlength{\textheight}{9.5in}
\setlength{\textheight}{10.0in}
%\setlength{\textheight}{10.5in}
%\setlength{\textheight}{11.0in}

%\setlength{\topmargin}{-1.05in}
%\setlength{\topmargin}{-0.65in}
%\setlength{\topmargin}{-0.25in}
%\setlength{\topmargin}{0in}
\setlength{\topmargin}{0.1cm}

\setlength{\oddsidemargin}{-0.5cm}
\setlength{\evensidemargin}{-0.5cm}

\setlength{\parindent}{0cm}
%\setlength{\parskip}{2ex}
\setlength{\parskip}{1ex}

\addtolength{\hoffset}{-0.5cm}
\addtolength{\voffset}{-2.5cm}

\renewcommand{\baselinestretch}{1.4}

%\makeindex

\setcounter{tocdepth}{2}
\setlength{\tabcolsep}{0.8mm}

%END OF PREAMBLE



